Remix: Rebalanced Mixup

Deep image classifiers often perform poorly when training data are heavily class-imbalanced. In this work, we propose a new regularization technique, Remix, that relaxes Mixup's formulation and enables the mixing factors of features and labels to be disentangled. Specifically, when mixing two samples, while features are mixed in the same fashion as Mixup, Remix assigns the label in favor of the minority class by providing a disproportionately higher weight to the minority class. By doing so, the classifier learns to push the decision boundaries towards the majority classes and balance the generalization error between majority and minority classes. We have studied the state-of-the art regularization techniques such as Mixup, Manifold Mixup and CutMix under class-imbalanced regime, and shown that the proposed Remix significantly outperforms these state-of-the-arts and several re-weighting and re-sampling techniques, on the imbalanced datasets constructed by CIFAR-10, CIFAR-100, and CINIC-10. We have also evaluated Remix on a real-world large-scale imbalanced dataset, iNaturalist 2018. The experimental results confirmed that Remix provides consistent and significant improvements over the previous methods.

==> OLD.tex <==
% \subsection{Theoretical Motivation}
% Inspired by the trade-off between the class margins, Cao \etal \cite{ldam} proved that if a binary classification task is separable (meaning that all the training examples are classified correctly), the optimal generalization error can be achieved by enforcing the below margins. (Please see \cite{ldam} for the exact proof.)

% \begin{align}
% \gamma_1 = \frac{C}{n_1^{1/4}}, \textup{ and } \gamma_2 = \frac{C}{n_2^{1/4}}
% \end{align} where $n_i$ denotes the number of data of class $i$ and $\gamma_i$ denotes the margin for class i. Note that the margin of an example $(x,y)$ is defined as: 
% \begin{align}
% \gamma(x,y) = f(x)_y - \max_{j\neq y} f(x)_j
% \end{align} and the margin for class $i$ is defined as: 
% \begin{align}
% \gamma_j = \min_{i \in S_j }\gamma(x_i, y_i) 
% \end{align}

% They use a soft margin loss to enforce the margins. We can't help but ask ourselves, are there any other regularizations to enforce the margins? We then investigated into the recent advanced regularizations including Mixup, Manifold Mixup and CutMix and found out that similar ideas could be integrated into them. We re-design the recent Mixup-based regularizations to form better margins for imbalanced datasets. Before we describe our method, we would first briefly introduce those advanced regularizations.




% \subsection{\imbmixup}
In this section, we show how Mixup is redesigned to \imbmixup\ and explain our core idea step by step. For ease of understanding, we first re-write the formulation of Mixup as below. 
\begin{equation}
\begin{split}
  \tilde{x} &= \lambda_x x_i + (1 - \lambda_x) x_j,\\
  \tilde{y} &= \lambda_y y_i + (1 - \lambda_y) y_j,
\end{split}
\end{equation}
\begin{equation}
  \lambda_y = \lambda_x  \\
\end{equation}
As we have shown in the preliminaries,  None of the above is designed for imbalanced datasets. To achieve our goal of enforcing better margins, the interpolation in the label space has to be shifted towards the minority class. We use the below example to explain what we mean by "shifting towards the minority class. For example, if a mixed sample that is generated with the weighted sum of a majority class sample $x_M$ and a minority class sample $x_m$ with the weight (0.7, 0.3) respectively, then instead of using the label of the weighted sum of the one-hot vector with the weight (0.7, 0.3) like Mixup, we may use (0.5, 0.5), (0.4, 0.6) or even (0.0, 1.0). 

To give a more formal definition of this example, we first analyze the four cases that will occur during mixing.  
\begin{equation*}
\begin{cases}
    \textbf{Case1: }x_i\in{M} $ and $ x_j\in{M}\\
    \textbf{Case2: }x_i\in{m} $ and $ x_j\in{m}\\
    \textbf{Case3: }x_i\in{M} $ and $ x_j\in{m}\\
    \textbf{Case4: }x_i\in{m} $ and $ x_j\in{M}\\
\end{cases}
\end{equation*}

% \begin{equation*}
% \begin{cases}
    
%     \textbf{Case1: }x_i\in{M} $ and $ x_j\in{m}\\
%     \textbf{Case2: }x_i\in{m} $ and $ x_j\in{M}\\
%     \textbf{Case3: } $otherwise$ \\
% \end{cases}
% \end{equation*}


$\mathit{M}$ denotes majority classes and $\mathit{m}$ denotes minority classes. Our method only focuses on mixed samples that are created under the case 3 or case 4, since our main goal is to be strict on majority class samples and less strict on minority class samples. Note that for a given class $i$, whether it is defined as a majority class or minority class is not determined by the number of data $n_i$, but the ratio of the given class and the other class (class j) that the interpolation is conducted with. For example, if $n_i$/$n_j$ is larger than a threshold $t$, then we consider class i to be a majority class and consider class j as a minority class. Vice versa, if $n_i$/$n_j$ is smaller than a threshold $1/t$, then class i is the minority class and class j is the minority class. If it's not the above cases, then we consider the class i and class j as balanced. In other words, "majority" and "minority" is a relative concept. Class $i$ might be a majority class to class $j$ but a minority class to class $k$. Based on the above definition, we can build a relation matrix $\mathbf{R}$ $\in \{0,1,2,3\}^{n \times n}$ where each element defines the relation of the given two classes and n denotes the number of classes.

The only challenge left now is how we determine $\lambda_y$ given $\lambda_x$. We already know that we need to shift $\lambda_y$ towards the minority classes. But the exact mechanism is not clear. After some empirical studies, we found that the following formulation works fairly well in general and provides flexibility in hyper-parameter tuning with $\tau$. 




\begin{equation}
\begin{split}
  \lambda_y = \lambda_x + offset(\lambda_x)
\end{split}
\end{equation}
where we define the offset function as follow:

\begin{numcases}{offset(\lambda_x) =}
     1-\lambda_x, & $\text{if } (x_i, x_j)\in$(M,m) and $ \tau > \lambda_x $; \\
     -\lambda_x, & $\text{if } (x_i, x_j)\in$(m,M) and $ \tau > 1-\lambda_x$;\\
     0, & $\text{otherwise}$.
\end{numcases}
where we define the offset function as follow:

% \begin{equation}
% \begin{split}
%   \lambda_y = F(\lambda_x)
% \end{split}
% \end{equation}
% where we define the function $F(\lambda_x)$ as follow:

% \begin{numcases}{F(\lambda_x) =}
%      1-\lambda_x, & $\text{if } (x_i, x_j)\in$(M,m) and $ \tau > \lambda_x $; \\
%      -\lambda_x, & $\text{if } (x_i, x_j)\in$(m,M) and $ \tau > 1-\lambda_x$;\\
%      0, & $\text{otherwise}$.
% \end{numcases}

One may consider the hyper-parameter $\tau$ as how much trade-off you want to make between a majority class and a minority class. Attentive readers may realize that using the same $\tau$ for various pairs of a majority class and a minority class implies that we want to enforce the same margin trade-off for those pairs which does not align with the optimal trade-off mentioned in section 3.1. The reason is that the optimal trade-off is proved under the assumptions of a binary linear classifier. When it comes to highly non-linear deep neural networks, The trade-off for multi-class problem is intractable to define. Hence, instead of defining $n$ number of $\tau$ for each pair of majority class and a minority class, we use a single $\tau$ for all pairs of them. Despite its simplicity, using a single $\tau$ is sufficient to achieve a better trade-off.

The proposed end-to-end training algorithm is shown in Algorithm~\ref{alg:final}. Consider training a neural network $f_\theta$ on a class-imbalanced dataset $\mathcal{D}$. Our proposed method attempts to make $f_\theta$ stricter on majority classes $M$ and be less strict on minority classes $m$ by mixed samples $\Tilde{x}$. During each training step,  if the interpolation is conducted between two majority classes or two minority classes, $\lambda_y$ is equal to $\lambda_x$. As a result, regular Mixup would be applied where both the input data and the one hot encoding of the labels would be mixed according to the $\lambda_x$ sampled from the beta distribution. If the interpolation is conducted between a majority class and a minority class and $\lambda_x$ is eligible, then the interpolation for labels would be be shifted towards the minority class based on the offset function. To give a straightforward explanation of why this would benefit learning with imbalance datasets, consider a mixed example $\Tilde{x}$ between a majority class and a minority class, the mixed samples include features of both classes yet we mark it as the minority class more. This force $f_\theta$ to learn that when there are features of a majority class and a minority class appearing in the sample, it should more likely to consider it as the minority class. This means that the classifier is being less strict to the minority class. Please see Section 4.7 for qualitative analysis. 


\begin{algorithm}[t]
\caption{Optimization with \imbmixup} \label{alg:final}
\begin{algorithmic}[1]

\Require Dataset $\mathcal{D} = \{(x_i,y_i)\}_{i=1}^n$. A parameterized model $f_\theta$
\State Define relation matrix \Comment For determining the majority-minority relation
\State Initialize the model parameters $\theta$ randomly
\For {$t=1$ to $T_0$}

	\State  ${(x, y)}\leftarrow \text{SampleMiniBatch}(\mathcal{D}, m)$  \Comment{a mini-batch of $m$ examples}
	\State  $(\hat{x}, \hat{y})\leftarrow \text{Shuffle}(x,y)$  \Comment{Create a shuffled batch MB}
% 	\State \ifthenelse{a}{b}{c}
    % \Comment{create a mixed batch}
    \For {$i=1$ to $m$}
        \State$(\tilde{x}_i, \tilde{y}_i) \leftarrow \text{\imbmixup}(x_i, y_i, \hat{x}_i, \hat{y}_i)$
    
    \EndFor
    \Comment{create a mixed batch}
    \State $\mathcal{L}(f_\theta) \leftarrow \frac{1}{m} \sum_{(\tilde{x},\tilde{y})\in MB}L((\tilde{x},\tilde{y});f_\theta) $ 
    
    \State $f_\theta \leftarrow f_\theta - \alpha\nabla_\theta \mathcal{L}(f_\theta)$ \Comment one SGD step
    \State Optional: $\alpha \leftarrow  \alpha/\tau$  \Comment anneal learning rate if necessary
    
\EndFor


\end{algorithmic}
\end{algorithm}


